Detecting Line Segments in Motion-blurred Images with Events

Making line segment detectors more reliable under motion blurs is one of the most important challenges for practical applications, such as visual SLAM and 3D reconstruction. Existing line segment detection methods face severe performance degradation for accurately detecting and locating line segments when motion blur occurs. While event data shows strong complementary characteristics to images for minimal blur and edge awareness at high-temporal resolution, potentially beneficial for reliable line segment recognition. To robustly detect line segments over motion blurs, we propose to leverage the complementary information of images and events. To achieve this, we first design a general frame-event feature fusion network to extract and fuse the detailed image textures and low-latency event edges, which consists of a channel-attention-based shallow fusion module and a self-attention-based dual hourglass module. We then utilize two state-of-the-art wireframe parsing networks to detect line segments on the fused feature map. Besides, we contribute a synthetic and a realistic dataset for line segment detection, i.e., FE-Wireframe and FE-Blurframe, with pairwise motion-blurred images and events. Extensive experiments on both datasets demonstrate the effectiveness of the proposed method. When tested on the real dataset, our method achieves 63.3% mean structural average precision (msAP) with the model pre-trained on the FE-Wireframe and fine-tuned on the FE-Blurframe, improved by 32.6 and 11.3 points compared with models trained on synthetic only and real only, respectively. The codes, datasets, and trained models are released at: https://levenberg.github.io/FE-LSD

==> README <==

August 26, 2015


IEEEtran is a LaTeX class for authors of the Institute of Electrical and
Electronics Engineers (IEEE) transactions journals and conferences.
The latest version of the IEEEtran package can be found at CTAN:

http://www.ctan.org/pkg/ieeetran

as well as within IEEE's site:

http://www.ieee.org/

For latest news, helpful tips, answers to frequently asked questions,
beta releases and other support, visit the IEEEtran home page at my
website:

http://www.michaelshell.org/tex/ieeetran/

Version 1.8b has a number of significant changes over the v1.8a release.
For a full history of changes, please read the file changelog.txt.
The most notable changes in this release include:

 1) Added new comsoc mode for the IEEE Communications Society.
    This mode (at present) only invokes the use of the newtxmath math fonts.
 
 2) Revised IEEEeqnarray column specifications to work with active " 
    (or other punctuation catcode changes) as with babel under the
    german or ngerman language modes. 
    Thanks to Stefan M. Moser for reporting this problem.

 3) Added \indexspace and other index related macros as newer versions of
    article.cls now do. These macros are needed to avoid an error when
    using the glossaries package.
    Thanks to Sebastian Nyberg for suggesting this change.

 4) Fixed odd/even page header font bug under compsoc mode and
    other page style code improvements.
    Thanks to Marco Paolieri for reporting this problem.

 5) Added hooks to allow for easy control of spacing above title.

 6) Added the \IEEEnoauxwrite command.
    Thanks to Sudarshan Mukherjee for suggesting this feature.


NOTE: Take care not to confuse the "comsoc" and "compsoc" class
options/modes as they are very different:

comsoc  ==> IEEE Communications Society
compsoc ==> IEEE Computer Society

The comsoc mode requires that an acceptable Times math font be available on
the LaTeX system. This requirement will be enforced by IEEEtran in comsoc
mode. Either the freely available newtxmath font by Michael Sharpe
http://www.ctan.org/pkg/newtx
(version 1.451, July 28, 2015 or later is recommended)
or the commercial MathTime font (e.g., mtpro2.sty) is acceptable.
See Section II-D (2.4) "Class Options - comsoc, compsoc, transmag" of
the IEEEtran HOWTO for more details.


Best wishes for all your publication endeavors,

Michael Shell
http://www.michaelshell.org/


********************************** Files **********************************

README                 - This file.

IEEEtran.cls           - The IEEEtran LaTeX class file.

changelog.txt          - The revision history.

IEEEtran_HOWTO.pdf     - The IEEEtran LaTeX class user manual.

bare_conf.tex          - A bare bones starter file for IEEE conference papers.

bare_conf_compsoc.tex  - A bare bones starter file for IEEE Computer Society
                         conference papers.

bare_jrnl.tex          - A bare bones starter file for IEEE journal papers.

bare_jrnl_comsoc.tex   - A bare bones starter file for IEEE Communications
                         Society journal papers.

bare_jrnl_compsoc.tex  - A bare bones starter file for IEEE Computer Society
                         journal papers.

bare_jrnl_transmag.tex - A bare bones starter file for IEEE Transactions
                         on Magnetics journal papers.

bare_adv.tex           - A bare bones starter file showing advanced
                         techniques such as conditional compilation,
                         hyperlinks, PDF thumbnails, etc. The illustrated
                         format is for an IEEE Computer Society journal paper.

***************************************************************************
Legal Notice:
This code is offered as-is without any warranty either expressed or
implied; without even the implied warranty of MERCHANTABILITY or
FITNESS FOR A PARTICULAR PURPOSE! 
User assumes all risk.
In no event shall the IEEE or any contributor to this code be liable for
any damages or losses, including, but not limited to, incidental,
consequential, or any other damages, resulting from the use or misuse
of any information contained here.

All comments are the opinions of their respective authors and are not
necessarily endorsed by the IEEE.

This work is distributed under the LaTeX Project Public License (LPPL)
( http://www.latex-project.org/ ) version 1.3, and may be freely used,
distributed and modified. A copy of the LPPL, version 1.3, is included
in the base LaTeX documentation of all distributions of LaTeX released
2003/12/01 or later.
Retain all contribution notices and credits.
** Modified files should be clearly indicated as such, including  **
** renaming them and changing author support contact information. **

File list of work: IEEEtran.cls, IEEEtran_HOWTO.pdf, bare_adv.tex,
                   bare_conf.tex, bare_conf_compsoc.tex, bare_jrnl.tex,
                   bare_jrnl_comsoc.tex, bare_jrnl_compsoc.tex,
                   bare_jrnl_transmag.tex
***************************************************************************


==> include/results/epe_compare.tex <==
\begin{table}[t!]
    \caption{The end-point error comparison of LOFT with or without FOA.}
    \label{tab:offset_epe}
    \vspace{-2mm}
    \renewcommand{\arraystretch}{1.2}
    \renewcommand{\tabcolsep}{4.0mm}
    \centering
    \begin{tabular}{ccc}
        \toprule
        Method      & LOFT  & LOFT w/ FOA\\
        \midrule
        Average EPE (pixel) & 5.26  & \textbf{4.94}\\
        \bottomrule
    \end{tabular}
    % \vspace{\fixedvskiptab}
    \vspace{-3mm}
\end{table}



==> include/results/foa_angle_set.tex <==
\begin{table}[t]
    \caption{F1-Scores of different rotation angle sets in the FOA module.}
    \label{tab:offset_rcnn_foa}
    % \vspace{\fixedvskiptab}
    \vspace{-2mm}
    \renewcommand{\arraystretch}{1.1}
    \renewcommand{\tabcolsep}{3.0mm}
    \centering
    \begin{tabular}{clc}
        \toprule
        Method                   & Rotation angle set  & F1-Score (\%) \\
        \midrule

        \multirow{4}{*}{LOFT w/ FOA}  
                        & $\{0\}$	                    & 61.78\\
                        & $\{0, \pi/2\}$	            & 63.83\\
                        & $\{0, \pi/2, \pi\}$	        & 63.95\\
                        & $\{0, \pi/2, \pi, 3\pi/2\}$	& \textbf{64.31} \\
        \bottomrule
    \end{tabular}
    % \vspace{\fixedvskiptab}
    \vspace{-3mm}
\end{table}



==> include/results/foa_share_parameter.tex <==
\begin{table}[t]
    \caption{Results of different network design choices of the FOA. Conv and FC mean the convolution and fully connected layers, respectively.}
    \vspace{-2mm}
    \label{tab:foa_share_parameter}
    \renewcommand{\arraystretch}{1.1}
    \renewcommand{\tabcolsep}{2.0mm}
    \begin{center}
    \begin{tabular}{lccc}
        \toprule
        Method                                  & Share Conv          & Share FC          & F1-Score (\%) \\
        \midrule
        
        \multirow{4}{*}{LOFT w/ FOA}     &  	-	        & -             & 63.84    \\
                                                 & \checkmark	    & -             & 63.22    \\
                                                 & -	            & \checkmark    & \textbf{64.31}   \\
                                                 & \checkmark	    & \checkmark    & 62.94  \\
        \bottomrule
    \end{tabular}
    \end{center}
    \vspace{\fixedvskiptab}
\end{table}

==> include/results/foa_vis.tex <==
\begin{figure}[!t]
    \renewcommand{\tabcolsep}{0.4mm}
    \renewcommand{\arraystretch}{0.7}
    \newcommand{\firstimage}{L18_104512_210416__0_1024}
    \newcommand{\secondimage}{shanghai_arg__L18_107160_219496__0_1024}
    \centering
	\begin{tabular}{ccc}
	
	\includegraphics[width=0.32\linewidth]{images/FOA_Vis/LOFT/\firstimage} &
    \includegraphics[width=0.32\linewidth]{images/FOA_Vis/LOFT_FOA/\firstimage} &
    \includegraphics[width=0.32\linewidth]{images/FOA_Vis/GT/\firstimage}
	\\
	\includegraphics[width=0.32\linewidth]{images/FOA_Vis/LOFT/\secondimage} &
    \includegraphics[width=0.32\linewidth]{images/FOA_Vis/LOFT_FOA/\secondimage} &
    \includegraphics[width=0.32\linewidth]{images/FOA_Vis/GT/\secondimage}
    \\
	\footnotesize{LOFT} & \footnotesize{LOFT w/ FOA} & \footnotesize{Ground Truth}
	\end{tabular}
	
% 	\vspace{-2mm}
	\caption{Qualitative comparison between LOFT and LOFT w/ FOA. Best viewed in color and zoomed-in view.}
	\vspace{-3mm}
	\label{fig:foa-vis}
\end{figure}

==> include/results/loft_foa_upper.tex <==
\begin{table}[t]
    \caption{The F1-Scores of roof and footprint extraction by using LOFT or Mask R-CNN.}
    \label{tab:offset_upper}
    % \vspace{\fixedvskiptab}
    \vspace{-2.5mm}
    \renewcommand{\arraystretch}{1.1}
    \renewcommand{\tabcolsep}{3.0mm}
    \centering
    \begin{tabular}{lccc}
        \toprule
        Method                                  & Roof (\%)         & Footprint (\%) & Gap (\%) \\
        \midrule
        LOFT w/ FOA                            & \textbf{67.25}	   & \textbf{64.31} & \textbf{2.94}   \\
        Mask R-CNN~\cite{Mask-R-CNN_2017_ICCV} & 67.10             & 58.12 & 8.98 \\
        \bottomrule
    \end{tabular}
    \vspace{-2mm}
    % \vspace{\fixedvskiptab}
\end{table}

==> include/results/loft_res.tex <==
\begin{table}[t]
    \caption{The influence of offset head on BONAI dataset (\%).}
    \label{tab:influence_offset}
    % \vspace{\fixedvskiptab}
    \vspace{-2mm}
    \renewcommand{\tabcolsep}{2.0mm}
    \renewcommand{\arraystretch}{1.1}
    \centering
    \begin{tabular}{lcccc}
        \toprule
        Method                        & F1-Score & Precision & Recall & AP$_{50}^B$\\
        \midrule
        Mask R-CNN~\cite{Mask-R-CNN_2017_ICCV}      			  & 58.12     & 59.26           & 57.03 & 45.80\\
        
        Mask R-CNN + Offset       	  & \textbf{61.78}    & \textbf{60.87}         & \textbf{62.72} & \textbf{50.10}\\
        \midrule
        PANet~\cite{PANet_2018_CVPR}                         & 58.06 & 59.26 & 56.91 & 45.30 \\
        PANet + Offset                & \textbf{62.15} & \textbf{61.33} & \textbf{62.99} & \textbf{49.90}\\
        \midrule
        HRNetv2-W32~\cite{HRNet_2019_arXiv}            & 60.81 & 61.20 & 60.42 & 50.10\\
        HRNetv2-W32 + Offset   & \textbf{63.16} & \textbf{62.31} & \textbf{64.03} & \textbf{52.00}\\
        \midrule
        CM R-CNN~\cite{HTC_2019_CVPR}            & 60.94 & 67.09 & 55.83 & 46.50\\
        CM R-CNN + Offset   & \textbf{63.73} & \textbf{68.29} & \textbf{59.74} & \textbf{48.70} \\
        \bottomrule
    \end{tabular}
    % \vspace{\fixedvskiptab}
    \vspace{-3mm}
\end{table}

==> include/results/main_results.tex <==
\begin{table}[t!]
    \caption{Quantitative comparison of the baselines and our methods on the test set of BONAI dataset. Bold and underline fonts indicate the best and the second best performances for each metric (\%).}
    % \vspace{\fixedvskiptab}
    \vspace{-2mm}
    \label{tab:main_results}
    \renewcommand{\arraystretch}{1.1}
    \renewcommand{\tabcolsep}{2mm}
    \centering
    \begin{tabular}{lcccc}
        \toprule
        Method                                      & F1-Score & Precision     & Recall & AP$_{50}^B$\\
        \midrule
        MAP-Net~\cite{MAP-Net_2020_TGRS}            & 56.92        & 58.01        & 55.93 & 30.30\\
        PANet~\cite{PANet_2018_CVPR}                & 58.06        & 59.26        & 56.91 & 45.30\\
        Mask R-CNN~\cite{Mask-R-CNN_2017_ICCV}      & 58.12        & 59.26        & 57.03 & 45.80\\
        HRNetv2-W32~\cite{HRNet_2019_arXiv} & 60.81 & 61.20 & \underline{60.42} & \underline{50.10}\\
        CM R-CNN~\cite{HTC_2019_CVPR}     & \underline{60.94}        & \textbf{67.09}        & 55.83 & 46.50 \\
        Ours     & \textbf{64.31}  & \underline{63.37} & \textbf{65.29} & \textbf{53.40}\\
        \bottomrule
    \end{tabular}
    %\vspace{\fixedvskiptab}
    \vspace{-2mm}
\end{table}


==> include/results/main_vis.tex <==
\begin{figure*}[!t]
    \renewcommand{\tabcolsep}{0.4mm}
    \renewcommand{\arraystretch}{0.50}
    \newcommand{\firstimage}{L18_104544_210392__0_1024}
    \newcommand{\secondimage}{L18_104512_210416__0_1024}
    \newcommand{\thirdimage}{L18_104536_210432__1024_0}
    \newcommand{\fourthimage}{shanghai_arg__L18_107192_219496__1024_1024}
    \centering
	\begin{tabular}{ccccc}
	
	\includegraphics[width=0.195\linewidth]{images/Comparison_Vis/MAP-Net/\firstimage} &
    \includegraphics[width=0.195\linewidth]{images/Comparison_Vis/Mask/\firstimage} &
    \includegraphics[width=0.195\linewidth]{images/Comparison_Vis/Cascade/\firstimage} &
    \includegraphics[width=0.195\linewidth]{images/Comparison_Vis/LOFT_FOA/\firstimage} &
    \includegraphics[width=0.195\linewidth]{images/Comparison_Vis/GT/\firstimage}
	\\
	\includegraphics[width=0.195\linewidth]{images/Comparison_Vis/MAP-Net/\thirdimage} &
    \includegraphics[width=0.195\linewidth]{images/Comparison_Vis/Mask/\thirdimage} &
    \includegraphics[width=0.195\linewidth]{images/Comparison_Vis/Cascade/\thirdimage} &
    \includegraphics[width=0.195\linewidth]{images/Comparison_Vis/LOFT_FOA/\thirdimage} &
    \includegraphics[width=0.195\linewidth]{images/Comparison_Vis/GT/\thirdimage}
	\\
	\includegraphics[width=0.195\linewidth]{images/Comparison_Vis/MAP-Net/\fourthimage} &
    \includegraphics[width=0.195\linewidth]{images/Comparison_Vis/Mask/\fourthimage} &
    \includegraphics[width=0.195\linewidth]{images/Comparison_Vis/Cascade/\fourthimage} &
    \includegraphics[width=0.195\linewidth]{images/Comparison_Vis/LOFT_FOA/\fourthimage} &
    \includegraphics[width=0.195\linewidth]{images/Comparison_Vis/GT/\fourthimage}
    \\
	\footnotesize{MAP-Net~\cite{MAP-Net_2020_TGRS}} & \footnotesize{Mask R-CNN~\cite{Mask-R-CNN_2017_ICCV}} & \footnotesize{CM R-CNN~\cite{HTC_2019_CVPR}} & \footnotesize{Ours} & \footnotesize{}Ground Truth
	\end{tabular}
	
% 	\vspace{-2mm}
	\caption{Qualitative comparison between the prior arts of BFE and our method on BONAI dataset. Best viewed in color and zoomed-in view.}
	\vspace{-3mm}
	\label{fig:offset-rcnn-vis}
\end{figure*}
